SecurePtrs: Proving Secure Compilation with Data-Flow Back-Translation and Turn-Taking Simulation

Proving secure compilation of partial programs typically requires back-translating an attack against the compiled program to an attack against the source program. To prove back-translation, one can syntactically translate the target attacker to a source one -- i.e., syntax-directed back-translation -- or show that the interaction traces of the target attacker can also be emitted by source attackers -- i.e., trace-directed back-translation. Syntax-directed back-translation is not suitable when the target attacker may use unstructured control flow that the source language cannot directly represent. Trace-directed back-translation works with such syntactic dissimilarity because only the external interactions of the target attacker have to be mimicked in the source, not its internal control flow. Revealing only external interactions is, however, inconvenient when sharing memory via unforgeable pointers, since information about shared pointers stashed in private memory is not present on the trace. This made prior proofs unnecessarily complex, since the generated attacker had to instead stash all reachable pointers. In this work, we introduce more informative *data-flow traces*, combining the best of syntax- and trace-directed back-translation in a simpler technique that handles both syntactic dissimilarity and memory sharing well, and that is proved correct in Coq. Additionally, we develop a novel *turn-taking simulation* relation and use it to prove a recomposition lemma, which is key to reusing compiler correctness in such secure compilation proofs. We are the first to mechanize such a recomposition lemma in the presence of memory sharing. We use these two innovations in a secure compilation proof for a code generation compiler pass between a source language with structured control flow and a target language with unstructured control flow, both with safe pointers and components.

==> capabilities.tex <==
% !TEX root = ./main.tex

As mentioned earlier, to be
able to realize compiler security in general,
a compiler relies on the availability of
a memory-isolation hardware feature.
Our compiler model relies on the
availability of a hardware
feature called hardware capabilities. 
To a first approximation, hardware
capabilities are an ISA-level
implementation of fat pointers, i.e., pointers
that carry bounds and possibly other information,
not just the address. This extra
information is maintained unforgeably by design thanks to a tracking
mechanism that a capabilities ISA enforces.
Unforgeability of the information of the fat
pointer means the fat pointer can be used not
only to protect against inadvertently buggy
accesses but also to protect against 
maliciously designed accesses. Some more
background on memory access control and
on capabilities is given in \Cref{capabilities-intro}.

Hardware capabilities is a feature that
disallows illegal memory accesses at
run-time.
The main advantage of hardware 
capabilities is that they
allow \emph{fine-grained} and \emph{dynamic} 
access control 
on memory, which
means that an arbitrarily small interval 
of the memory
of a compartment (i.e., a program part) can be shared 
with another compartment \emph{at run time}.
Being arbitrarily small thus enables a compartment
to intentionally share its own memory
with other compartments while at the same time 
enabling it to faithfully
realize/enforce the \emph{principle of least privilege}:
a callee compartment gets the permission to access only 
the memory
locations that the caller compartment expects it to access
and nothing more.



According to reports by both Microsoft~\cite{microsoft-memory-safety} 
and the Chromium team~\cite{chromium-memory-safety},
	roughly 70\% of all serious security bugs reported are memory
	management and memory safety bugs. This class of bugs has been
	dominating the statistics for decades. As a consequence, it has gradually
	become common
	practice in many software engineering processes to use tools (like dynamic
	analysis and fuzzing) that try to find these bugs. These tools
	are effective in finding bugs, but they are not a \emph{guarantee} that
	the program is bug-free. Thus, when the risk of exploiting a memory
	safety bug is very high, there is still need for complementary approaches that
	\emph{ensure} either that the program is bug free or that \emph{at run-time}, 
	all illegal memory accesses will be \emph{disallowed}.


To disallow all ``illegal'' memory accesses at run-time, one needs to
ensure that every memory access is preceded by a check 
of whether this
access is legal. 
This check can be, for example, introduced by the 
compiler.
However, if the legality check is introduced by the compiler, then there
still remains the problematic
scenario in which a \emph{partial program}---despite having been compiled with 
these checks---gets nevertheless
linked with a context that was not compiled the same way, i.e.,
a context whose memory accesses are not checked for legality. 
Or it could even be the
case (as in the implementation of many crypto libraries) that the context
is (partly) written directly in assembly, and thus there is no way for it
to benefit from such compiler-introduced checks. A memory safety bug in such
an assembly-level context will affect the behavior of a partial program that
runs in this
context, and can potentially invalidate the assumptions/premises of some 
invariants or
guarantees that the author of the partial program has proved or thought about.
For example, a spatial memory safety bug in the context can mean that the
context will read/overwrite some memory location that the author of the
partial program has intended
to keep private (i.e., has intended to never share with the context).
This private memory can hold data whose confidentiality or integrity
is sensitive, but the compiler-introduced checks will not help enforce this
confidentiality or integrity guarantee against the buggy context code
because, clearly, the compiler alone has no control over code that it does not
generate (the context's code) and thus cannot alone solve the memory access
control problem.

So, instead of outsourcing the memory access control problem to the
compiler alone, one old approach called
\emph{capability machines} aims to solve this
problem at the bottom of the software stack, i.e., 
at the instruction-set-architecture (ISA) level
(Capability machines have been revived in recent years by the CHERI
 project~\cite{cheriageofrisk,cheriisatech,chericompartment,cheriprogrammers} that brought forth a 
 modern RISC-V-based implementation). 
 At the ISA level, the basic
memory operations (loads and stores) get their semantics. In a capability
machine, the legality checks (preceding a memory operation) are built into the
semantics of these memory-accessing instructions.
Therefore, regardless of how the assembly or machine code was produced,
a check will take place upon the execution of any load or store instruction.
However, clearly, one needs to ensure that the legality check mentioned above is performed 
against the correct authoritative information, which
is a language design problem.

For spatial memory safety checks, this 
information is the bounds of a certain memory region that 
represents, say, an
array in the source language. This authoritative information is 
program specific, and has to originate from the compiler, 
the linker and the
loader. The compiler collects---from
the program text---symbols representing the sizes of 
variables, arrays, and
structs. The linker combines symbols from different program parts. 
And finally, the loader is responsible for 
placing concrete addresses in registers and in the instructions that address the
memory. But crucially, the loader also places bounds information that
governs the partitioning of (the statically-allocated) 
memory among the
different program parts.

In a capability machine, these concrete addresses and bounds information are not
mere integers (as they would be in
a conventional ISA). Instead, both the
address and the bounds information in a capability machine are collected together
in a separate run-time type called a capability.
From the fields of a capability type, one can derive a conventional integer
address, but the other way around is not possible:
a capability value cannot be derived from an arbitrarily computed integer.
To derive a capability, one has to already start with a "bigger" capability.
This property (the impossibility of constructing a capability out of thin
air) is referred to as capability unforgeability. In a capability machine,
the ISA is designed to ensure capability unforgeability. And higher up in the
software stack, trusted programs like the loader and the memory allocator
hold universal capabilities, and are responsible for keeping them private
and for deriving smaller capabilities as needed.

Circling back to the scenario where a partial program is linked with a
buggy context that attempts to access its private memory, we can now rely
on the loader and on an architecture-level capability system to disallow
such an access: the loader will just do its conventional role of allocating
disjoint memory regions to the partial program and the context. However,
the disjointness now is \emph{enforced} by the fact that each program part
gets only a capability on the data segment that it defines, and not a capability
on the whole address space. When a program part calls another part, what happens
under the hood in a capability architecture is that the semantics of "call"
relies on kernel support (a trusted call stack) to hide the caller's 
capabilities. Moreover, the "call" semantics employs
a sealing/unsealing mechanism to ensure the callee gets the capability
it needs without having to trust the caller with holding and passing that
necessary capability. The caller holds just a sealed version of an entry-point
capability, and
the semantics of the call instruction ensures that two things happen only
atomically: unsealing of the capability and setting the program counter to the
entry point that is meant to use this capability. Therefore, only the code at 
this entry point can benefit from the authority that the entry-point capability
prescribes. And only this code can use it to derive more (smaller) capabilities.
The caller that holds just the sealed version cannot benefit from its authority
nor use it to derive any more capabilities.
Thus, thanks to a careful design of this call mechanism, and to the loader and
allocator ensuring disjointness of the capabilities that they derive for 
different memory regions, a partial program intuitively should be able to
interact safely with any context.

This intuition that capabilities can enable a 
\emph{partial}
program to interact safely with any context is the
motivation for relying on capabilities to build 
compilers that both support dynamic memory sharing
and that are provably secure
because the compiler security
theorems we are interested in are of the form 
``\emph{if a partial source program is secure against
all source contexts, then its compiled version also
is secure against all target contexts}''.

==> memory-sharing-interaction.tex <==
% !TEX root = ./paper.tex

%\aek{TODO: Fix this section.}
%\aek{Refactor this subsubsection out as a subection
%that precedes \autoref{sec:keyideas-proof-strategy}.
%In fact, introduce a \textbf{technical preliminaries} 
%subsection
%even before talking about the traces and the trace
%relation. The preliminaries subsection will need to
%mention values, addresses, memory, path in a memory,
%and value unforgeability (talk about path in the
%memory as the way to construct unforgeable
%values). and possibly also
%the reduction relation. (Maybe this preliminaries 
%section should even come before 
%\autoref{sec:keyideas-example}.)
%After having refactored out this subsubsection, make 
%sure to adapt the narrative of 
%\autoref{sec:keyideas-proof-strategy}.
%}
With memory sharing, components can interact with
each other by reading from and writing to memory
that was previously shared. These interactions need to
be captured on the trace.
Thus, our interaction traces $t$ disclose more 
information about the program state than the traces
of \cite{Abate:2018:GCG:3243734.3243745}, 
namely, ours now show a snapshot of the contents of
the memory locations that have been shared among
components.
%The source language of 
%\cite{Abate:2018:GCG:3243734.3243745} allowed only
%primitive values to be passed as arguments to
%cross-component calls (and returns). They achieved this
%restriction by means of a run-time check that would
%prevent a function call from receiving any memory 
%pointer as an argument.
%Clearly, this is a restrictive programming model, e.g.,
%it does not admit functions like 
%\src{populate\_partner\_ads} in our example from
%\autoref{sec:background-example}.
%As a result of this restrictive model of interaction
%between components, 
We will refer to the interaction traces without
memory sharing as $e_{\mi{no\_shr}}$:
\begin{align*}
e_{\mi{no\_shr}} ::=
\mathtt{Call}~\mathit{c_{caller}~c_{callee}.f(v)}
\mid
\mathtt{Ret}~\mathit{c_{prev}~c_{next}~v}
\end{align*}
The call and return events both record the component
%(i.e., module)\ch{Good. It would be good to always call these components.
%  IIRC sometimes it's called module now in abstract and intro.
%  Also very often the text calls things ``program parts'', but
%  it's unclear what those are. Sets of components?}
%\aek{yes, a program part is a set of components}
ids (lowercase $c$) corresponding to the source and 
destination of the call/return. 
They also record the argument ($\mathit{v}$), which is
restricted to be a primitive value (i.e., no locations).
%This information sufficed in~\cite{Abate:2018:GCG:3243734.3243745}
%to capture all of the
%observable behavior of a component. 
But with memory sharing,
interaction traces allow a value $v$ to be either a primitive
value or a memory location $l$, and
record a snapshot of
the \emph{shared-so-far} memory on calls and returns
because in a sequential model, calls and returns are
the points at which the shared content becomes
observed. 
%\dg{Why?}
This idea is not new. Recording a snapshot of
the shared memory at component-crossing events
is known~\cite{9249fdc52dd3414e83b2e3f9a89cb117,capableptrs} 
to be the \emph{fully-abstract} trace-based
representation
of the observable behavior of a program.
Here is the alphabet of our trace events (the extra 
information exposed---compared
to~$e_{\mi{no\_shr}}$---is \underline{$\mathit{underlined}$}):
\begin{definition}[Memory-sharing trace events $e$]
	\label{def-mem-sharing-trace-event}
	\begin{align*}
	e ::=
	\mathtt{Call}~\mathit{\underline{Mem}~c_{caller}~c_{callee}.f(v)}
	\mid
	\mathtt{Ret}~\mathit{\underline{Mem}~c_{prev}~c_{next}~v}
	\end{align*}
\end{definition}
%\aek{Try to
%	express both \textbf{NO\_WRITE} and
%	\textbf{SIMULT\_UPD} more formally, i.e., use them
%	to show the benefit of the
%	enriched trace alphabet that mentions the shared
%	memory.}

With these memory-sharing aware events, we can 
specify formally what it means for a trace $t$
to comply with the property \textbf{NO\_WRITE}.
We will write a memory \mi{Mem}
as a partial map of locations $l$ to values $v$ (which 
themselves can be locations),
and we will suppose there is a partial function
$\mathtt{find\_matching\_ret}$ that given a $\mathtt{Call}$
event and the rest of the trace, finds in
the rest of the trace the $\mathtt{Ret}$ event that matches the
given $\mathtt{Call}$ if one exists.

\begin{example}[The safety spec \textbf{NO\_WRITE}]
\label{example-NO-WRITE-spec} 
Suppose $l_\mi{balance}$ is the memory location allocated
for the variable \src{user\_balance\_usd}, and suppose
$c_\mi{main}$ denotes the component that calls the function 
\src{set\_ads\_image}, which is implemented by $c_\mi{setter}$.
\begin{align*}
&\textbf{NO\_WRITE}(t) \defeq\\
&\forall t_1\ e_\mi{call}\ t_2\ \mi{Mem_1}\ 
\mi{Mem_2}\ l.\\ 
&t = t_1\ \texttt{++}\ [e_\mi{call}]\ \texttt{++}\ t_2 \implies\\
&e_\mi{call} = \mathtt{Call}~\mathit{Mem_1~c_{main}~c_{setter}.set\_ads\_image()} \implies\\
&\mathtt{find\_matching\_ret}(t_2, e_\mi{call}) =\\ 
&\ \ \ \ \ \ \  \mathtt{Ret}~\mathit{Mem_2~c_{setter}~c_{main}.\mi{void}} \implies\\
&\mi{Mem_1}(l_\mi{balance}) = \mi{Mem_2}(l_\mi{balance})
\end{align*}
\end{example}
The spec above makes sure that the value of the variable
\src{user\_balance\_usd} before the call to the function
\src{set\_ads\_image} is the same as its value at the point
when the function returns.

%\Cref{example-NO-WRITE-spec} illustrates the benefit of 
%the memory-sharing trace alphabet
%(\Cref{def-mem-sharing-trace-event}) in expressing invariants
%on the shared memory. However, in 
Next, we explain that the alphabet of
\Cref{def-mem-sharing-trace-event}
of interaction traces even with a snapshot of the shared memory
is too abstract for the purpose of \emph{proving}
a back-translation lemma 
(like \Cref{lemma-abateetal-backtrans}).

%\dg{There is a problem here. The previous seems to suggest that the
%  reason we want shared memory on the trace is to be able to express
%  safety properties of programs. This begs the obvious question: Is
%  this the only criterion for deciding what is on the trace? It
%  doesn't seem to be. I would have expected that capturing all
%  interactions is what we want.}


==> old-content.tex <==
% !TEX root = ./paper.tex

\section{Introduction}

\begin{itemize}

\item Motivation

\item Contributions and outline

\end{itemize}

% Imperative ``call by value'' and adding ``call by name'' -- CH: ha?

\ifdraft
\clearpage
\fi

\section{Background}

\ch{More appropriate name for this section seems ``random leftovers''?}

\rb{TODO: Sometimes ``component'' may have been written instead of
``compartment'', check and correct if necessary. Also using ``original'' too
much to refer to the starting compiler and proofs.}

\subsection{A Simple Example}

Consider a simple imperative language with pointers that structures programs into
collections of modules. Each module is a collection of functions as well as
declarations of external function signatures on which the module relies.
Finally, each function in a module can be either public or private. All
functions can be called anywhere inside their module, but only public functions
can be called from other modules.

Based on this programming model, take a program
that relies on an externally provided library:

\begin{center}
\begin{lstlisting}
module View {
  public char* get_username() { /* ... */ }
  public char* get_password() { /* ... */ }
}

module Model {
  public char* get_user_data { /* ... */ }
}

module Controller {
  import char* Model.get_username();
  import char* Model.get_password();
  import int Lib.validate(char* input);
  int secret = 42;
  private int execute() {
    
  }
}
\end{lstlisting}
\captionof{figure}{Test}
\end{center}
%% \vspace{5pt}

{\em partial program}

Check password?

One way to represent program behaviors is as {\em traces} of events produced
during the execution of a program. A possible choice is to record the {\em
interactions} between different program modules, which are directly related to
function calls. In particular, we are interested in instances where a function
{\em calls} a public function defined in a different module or {\em returns} to
the function that called it from a different module. We refer to such traces of
cross-module calls and returns as {\em {\noninftraceTerm}s}.

\rb{Some illustration on the example. For example, two calls to the same
function, one of which modifies previously shared memory, which may have already
been validated or assumed to be unchanged by the caller.}

\rb{A benign version of a library.}

\begin{center}
\begin{lstlisting}
module Lib {
  int *copy = NULL;
  public x name(int *data) {
    if (data != NULL) { (*data)++; }
    copy = data;
    data ...
  }
}
\end{lstlisting}
\captionof{figure}{Test}
\end{center}
%% \vspace{5pt}

\rb{A malicious version of the library, represented in the source here.}

\rb{Low-level attackers, invariants.}

\rb{Secure compilers, safety properties, some things preserved, transition to
memory safety, extensions to memory model (later?).}

\subsection{\ldots}

%% \rb{How much should we rely on definitions vs. inlined explanations of concepts?
%% Match to audience.}

Goal: a proof of robust safety with fine-grained memory sharing.

\ifdraft
\clearpage
\fi

\section{Key Ideas}

\ch{This section could be called ``beating around the bush for many pages and
  maybe eventually getting to the key ideas buried down in a sea of random ideas ''.}

\begin{itemize}

\item Example(s) -- additional?

\item Basic proof overview. \rb{Make some points at basic level, maybe some
comparisons if the level of detail is right, later go into more.}

\item Three basic adaptations

\end{itemize}

The end result will be a technique that is much simpler than other work in this
domain -- why? Comparisons. \rb{Where to place these? We'll see\ldots}

\rb{We know we can go beyond robust safety. But, first proof of robust safety
with memory sharing?}

We want realism!\ch{with simple toy languages and compiler?}

\rb{Needs better subsectioning and naming}

\subsection{Secure Compilation}

\ch{bombastic}%
The quintessential notion of {\em compiler correctness} is defined in terms of
the familiar idea of a compiler $\downarrow$ that translates from a source
language \src{S} to a target language \trg{T}, both defined by a trace-producing
semantics, respectively \src{\sem} and \trg{\sem}. The standard specification of
correct compilation is stated as a {\em trace refinement}: for any whole source
program \src{W}, if its compilation can produce a trace \com{t} with respect to
the target semantics, then the same trace can be produced by the original
program with respect to the source semantics.
%
$$
\forall \src{W}.~t.~ \cmp{\src{W}} \trg{\sem} t \Rightarrow \src{W} \src{\sem} t
$$

\rb{Notes on notation. Refer to these criteria by name in this discussion? Add
$=$ to standard criteria?}

Because the implication goes from the target language to the source one,
so in the opposite direction to compilation,
this property can be referred to as {\em backward} compiler
correctness. Under certain conditions, it is possible to prove the opposite
direction, called {\em forward} compiler correctness, which says that any trace
produced by \src{W} is also produced by $\cmp{\src{W}}$. Taken together, these
two properties imply that the set of observable behaviors of a program is
unaltered by compilation.

Compiler correctness guarantees that the compiled code preserves the
abstractions and invariants established at the source level, but in its basic
form applies only to the compilation of whole source programs. More generally, a
program \src{W} may be structured as a collection of components organized as
separate {\em partial programs}. In practice, each component is compiled
independently from all others and a {\em linker} assembles a whole target
program from the resulting target components. In some cases, a {\em separate
compilation} result can strengthen basic compiler correctness to cover this
scenario.\ch{I guess you'll need this in your proof, no?}

Once the door is open to partial programs, the security problem becomes
apparent. While a good source language can provide facilities for writing
well-behaved programs, these properties are generally not preserved when the
compiled programs are linked against arbitrary target code, such as externally
provided libraries. Indeed, a low-level adversary could break security
properties and invariants established at the source level, rendering correct
compilation useless. The idea behind a {\em secure compilation chain} is to
protect compiled source programs in such a way that certain classes of security
properties are preserved in the target.

\ch{Introducing full abstraction (especially formally, but also in general)
  seems to me a useless detour.}

Until recently \rb{and still?}, the study of the protection of source-level
abstractions against adversarial target code has centered on {\em full
abstraction} \cite{Abadi99, MarcosSurvey}: the preservation and reflection of
contextual equivalence. A low-level adversary is usually represented as a {\em
context} that turns a partial program into a whole one. In the setting of
trace-producing semantics, two (possibly partial) programs \com{P_1}
and \com{P_2} are considered contextually equivalent, written $\approx_C$, if,
for any context \com{C} with which they can be linked to become whole programs,
the two programs produce the same traces.
%
$$\begin{multlined}
\forall \com{C}.~ \com{t}.~ \com{C \hole{P_1} \sem t \Leftrightarrow C \hole{P_2} \sem t}
\end{multlined}$$

Then, the security-relevant direction of full abstraction (i.e., preservation)
requires that, for any pair of programs that are contextually equivalent in the
source language, their compilations remain contextually equivalent in the
target.
%% \rb{And fix notation, in particular to avoid confusion with later
%% relations.}
%
$$\begin{multlined}
  \forall\src{P_1}.~\src{P_2}.~ \src{P_1 \approx_C P_2} \Rightarrow
  \trg{\com{\cmp{\src{P_1}}} \approx_C \com{\cmp{\src{P_2}}}}
\end{multlined}$$
%% \criteria{\oep}{oep}:

Note that contextual equivalence is a very strong requirement: it forces a
compilation chain to preserve {\em all} program interactions, including many
that may not be relevant for security. On the one hand, this need to account for
and harmonize differences between the source and target languages can lead to
inefficient compilers. On the other, this complexity can produce long and
difficult proofs, making them difficult to scale to rich languages, and
hindering the verification of fully abstract compilation chains to the highest
level of assurance, i.e., by means of mechanized proofs.

As a useful and practical alternative to full abstraction, a secure compilation
chain may endeavor to achieve {\em robust satisfaction} (i.e., against
adversarial contexts) of many different classes of security
properties \cite{AbateBGHPT19}. In particular, {\em safety properties} are an
attractive goal because they stand at a sweet spot between expressivity and ease
of satisfaction relative to other robust criteria.

A trace property is a safety property iff, for any finite or infinite
trace \com{t} that violates the property, there exists a {\em finite
prefix} \com{m \leq t} of that trace that also violates it.
\ch{Unclear what's the connection between the above and the below.
  Could consider showing both RSP and RSC and claiming they are equivalent,
  with a reference to \citet{AbateBGHPT19}}
The corresponding
criterion for secure compilation is {\em robustly safe compilation}
(\rsc) \cite{PatrignaniG18}.\ch{Wrong citation. They define something a bit
  different in a setting that was quite different.
  Your RSC below is from \citet{AbateBGHPT19}}
%
It states that, given any source program \src{P},
if the result of compiling it and linking it with an arbitrary target
context \trg{C_T} produces a finite trace prefix \com{m}, then one can find a
source context \src{C_S} that produces the same trace prefix when linked with
the original program.
\rb{Prefix vs trace squiggly? Overload notation and indicate so?}
%
$$\begin{multlined} \forall\src{P}.~ \forall\trg{C_T}.~ \forall
  m.~ \trg{C_T\hole{\com{\cmp{\src{P}}}}} \mathrel{\trg{\sem}} m \Rightarrow
\exists \src{C_S}\ldotp \src{C_S\hole{P}} \mathrel{\src{\sem}} m
\end{multlined}$$
  %% \criteria{\pf{\rsp}}{pfrsp}:\quad


\rb{This is the criterion we choose to adapt to our setting. Connect to existing
compiler, next part.}

\subsection{Memory Sharing}

\ch{This section has nothing to do with its title}

\rb{Not clear to me whether the outline of the proof should be given upfront
for the no-sharing case and particularized later, or whether memory sharing
should be discussed first, followed by its effects on the proof.}

The potential of \rsc has been effectively harnessed to build at least one
realistic\ch{I would definitely not call that compiler realistic}
secure compilation chain with fully mechanized
proofs \cite{AbateABEFHLPST18}. The \rscdcmd secure compiler (which we name here
after its security property) adopts {\em compartmentalization} as a flexible and
practical protection mechanism, adding language primitives to structure
applications as collections of compartments and specify their privileges. This
compilation chain refines the base \rsc criterion in two ways.\ch{None of these
  ways are relevant for the current work though. Are they? Our language is safe,
  so neither Mutual Distrust nor Dynamic Compromise is a concern for us.
  So this is all another big detour to explain complications that seem
  irrelevant here. How about instead explaining a simpler projection of that
  proof to safe languages?}

\begin{enumerate}

\item {\em Mutual Distrust (MD):} Source and target programs are typed via a
notion of {\em interface}: a set of the components defined by the program, and
for each component a set of exported procedures (which other components may
call) and a set of imported procedures (defined in other components, and which
the component may call). Programs are only allowed to interact as prescribed by
their interfaces, and from these arise natural definitions of linkability
between programs, whole programs, etc.\ch{What you say is true, but I don't
  see what the connection is to Mutual Distrust, which is about not knowing
  in advance which components are trusted and which are compromised.}

\item {\em Dynamic Compromise (DC):} Programs written in unsafe source languages
may become compromised by an attacker {\em and also} by ``shooting themselves in
the foot,'' i.e., triggering undefined behavior. An unsafe component may become
compromised during execution, but still enjoys source-level guarantees until
that moment. Moreover, if the program is linked with a well-behaved context yet
becomes compromised, it is possible to absolve the context and {\em blame} the
program for the misbehavior.

\end{enumerate}

The resulting criterion, {\em robustly safe compilation with dynamic compromise
and mutual distrust} (\rscdcmd), decorates the source program with an
interface \com{I_P} and both contexts with a shared interface \com{I_C}.
Moreover, it presumes that the source context \src{C_S} produced to simulate
\trg{C_T} can be guaranteed to \ch{be? }safe. Because the source program \src{P} is
possibly unsafe, the trace \com{t'} produced by \CsP may either be the expected
extension of \com{m}, or an early termination of a prefix of \com{m} due to
undefined behavior, which could then be pinned on the program, \com{t'
{\prec_{I_P}} m}.
\rb{Capitalize criteria, etc.}
\rb{Tweaks: quantified on \com{t'} instead of inlining back-translation, used
plugging notation instead of unions. Change?}
\rb{These formulas can also be given headers, references, etc.}
%
\[\arraycolsep=1pt
\begin{array}{rl}
\forall \src{P} {:} \com{I_P}.~ \trg{C_T}{:}\com{I_C}.~ & \com{t}.~
  \trg{C_T\hole{\com{\cmp{\src{P}}}}} \mathrel{\trg{\sem}} t \Rightarrow
  \forall \com{m{\leq}t}.~\\
  \exists \src{C_S} {:} \com{I_C}.~ & \com{t'}.~ \src{C_S\hole{P}} \mathrel{\src{\sem}} t'
  \wedge \com{(m {\leq} t' \vee t' {\prec_{I_P}} m)}
\end{array}
\]

% Original
%% \[
%% \begin{array}{l}
%% \forall P {:} I_P.~ \forall C_T{:}I_C.~ \forall t.~
%%   (C_T \cup \cmp{P}) {\rightsquigarrow} t \Rightarrow
%%   \forall m{\leq}t.~\\\quad
%%   \exists t'.~ (\{\back{(m,I_i)} \,|\, I_i \in I_C \} \cup P) {\rightsquigarrow} t'
%%   \wedge (m {\leq} t' \vee t' {\prec_{I_P}} m)
%%   .
%% % \text{where }\back{(m,I_C)} = \{\back{(m,I_i)} ~|~ I_i \in I_C \}
%% \end{array}
%% \]

The criterion comes equipped with a generic proof technique predicated on a
small number of assumptions, all shown in \autoref{fig:rsc-dc-md-proof}. The
technique is applicable to any compilation chain that satisfies them. To these
must be added a foundational requirement on execution traces, which must contain
enough information to recover the history of interactions between components,
i.e., the sequence of cross-component calls and returns.
\rb{Source language may be unsafe, target is assumed to be safe.}

\begin{figure*}
\centering
\input{proof-diagram}
%% \vspace{-0.8em}
\vspace{5pt}
\caption{Outline of the generic proof technique for \rscdcmd}
\label{fig:rsc-dc-md-proof}
\end{figure*}

The proof proceeds as follows. It starts from the source program of
interest \src{P}, which compiled and linked with an adversarial
context \trg{C_T} produces a finite trace prefix \com{m \leq t}. The first
assumption posits the existence of a {\em back-translation} function which,
given a trace prefix \com{m} produced by a target program-context
pair \trg{C\hole{P}} and their joint interface \com{I_P \cup I_C}, generates a
compatible source program-context pair that produces \com{m}.
\rb{Interface union notation? Maybe use holes to denote which is which?}
\rb{Stipulate this is restricted to ``well-defined traces''. Notation?}
%
%% Here, pairs are used instead of plain whole programs to express the requirement
%% that back-translation must be {\em horizontally compositional}, i.e., it can be
%% split into the part that simulates \trg{P} and the part that simulates \trg{C}.
%
\[\arraycolsep=1pt
\begin{array}{rl}
\exists \com{\uparrow}.~ &
\forall \trg{P_T} {:} \com{I_P}.~
        \trg{C_T} {:} \com{I_C}.~
        \com{m}.~
        \trg{C_T\hole{P_T} \mathrel{\sem} \com{m}}
\Rightarrow \\
& \com{(m, I_P \cup I_C)\uparrow {:} (I_P \cup I_C) \mathrel{\src{\sem}} m}
\end{array}
\]

Here, pairs are used instead of plain whole programs to express the requirement
that back-translation must be {\em horizontally compositional}, i.e., it can be
split into the part that simulates \trg{P} and the part that simulates \trg{C};
call the resulting pair \src{C_S\hole{P'}}. This source context \src{C_S} will
be used to instantiate the first existential in the goal. The second assumption
is a variant of {\em forward compiler correctness} with support for separate
compilation and undefined behavior. It says that, if a source program-context
pair \src{C\hole{P}} produces a well-defined trace \com{m}, then the result of
compiling program and context separately and linking them produces \emph{m} too.
\rb{Defined trace below. Focus on more generic linking rather than holes?}
%
$$\begin{multlined}
\forall \src{P}.~
        \src{C}.~
        \com{m}.~
        \src{C\hole{P} \mathrel{\sem} \com{m}}
\Rightarrow
\trg{\com{\cmp{\src{C}}}\hole{\com{\cmp{\src{P}}}} \mathrel{\sem} \com{m}}
\end{multlined}$$

From here it follows that
\trg{\com{\cmp{\src{C_S}}}\hole{\com{\cmp{\src{P'}}}}} also produces \com{m}.
The third assumption, {\em recombination},\ch{I still prefer calling this
  recomposition, like we already called it in the CCS paper (see Fig 3).}
%
takes two program-context pairs
defined on the same interfaces (here \trg{C_T\hole{\com{\cmp{\src{P}}}}} and
\trg{\com{\cmp{\src{C_S}}}\hole{\com{\cmp{\src{P'}}}}}), and which produce the
same trace (here \com{m}), and concludes that the parts are {\em
interchangeable}. That is, because \com{m} can be partitioned into program-side
and context-side interactions, and because both programs and both contexts
produce exactly the same interactions, each can be substituted for the other
without observable differences.
\rb{A special case of contextual equivalence, in a sense.}
%
\[\arraycolsep=1pt
\begin{array}{rl}
\forall & \trg{P_1 ~ P_2} {:} \com{I_P}.~
          \trg{C_1 ~ C_2} {:} \com{I_C}.~
          \com{m}.~ \\ &
\trg{C_1\hole{P_1} \mathrel{\sem} \com{m}} \Rightarrow
\trg{C_2\hole{P_2} \mathrel{\sem} \com{m}} \Rightarrow
\trg{C_2\hole{P_1} \mathrel{\sem} \com{m}}
\end{array}
\]

Consequently, \trg{\com{\cmp{\src{C_S}}}\hole{\com{\cmp{\src{P}}}}} also
produces \com{m}. The fourth assumption is standard (backward) {\em compiler
correctness}, again with separate compilation and undefined behavior. This
differs from compiler correctness for safe languages in that, even
though \com{m} must be well-behaved (it is produced by a target program), the
compiler could have refined undefined behavior present in the source. For this
reason, there are two options: either \com{m} is a prefix of the source trace,
or the source trace terminates prematurely due to undefined behavior.
\rb{Not sure this is as clear as the others.}
%
$$\begin{multlined}
\ldots
\end{multlined}$$

Call \com{t'} the trace produced by \src{C_S\hole{P}} in the source and use it
to instantiate the second existential. Compiler correctness almost gives the
conclusion. All that remains is using the fifth and last assumption, using
dynamic compromise to {\em blame} the program in the case that undefined
behavior occurs.
\rb{Pull explanation from DC above?}
%
$$\begin{multlined}
\ldots
\end{multlined}$$

\subsection{A Generic Proof Technique}

\rb{Now ``Memory Sharing'', ``Key Adaptations'', etc.}
\ch{So this section has nothing to do with its title either.}

\ch{Fortunately, it's getting a bit closer to the key ideas ... or at least some
  ideas, although it's very unclear from the writing which ones are the key
  ideas in a sea of random ideas. Before writing a proper key ideas section
  it would definitely help to think much harder what are the key ideas,
  and there can only be a few of those, not one hundred.}

The original instance of the \rscdcmd proof technique is a simple,
non-optimizing compiler between a small but expressive imperative language which
models the kernel of a language like C, and a core assembly language which
models the kernel of a RISC architecture as an abstract machine. Both languages
are enriched with compartmentalization primitives, used to express programmer
intent at the source level, and to keep enforcement relatively abstract at the
target level.
\rb{More about this? Buffers, procedures, pointers\ldots Later concretization
of enforcement by various backends.}

In that work, traces correspond exactly with sequences of cross-compartment
calls and returns, each recording the origin and destination components,
destination procedure and passed arguments in the case of calls, and returned
values in the case of returns. Each compartment has its own private memory
space, and {\em no sharing} is allowed: the passing of values back and forth
during calls and returns is the only means of communication between
compartments, and pointer passing is forbidden. Here, we generalize that line of
work to encompass the much more challenging setting with fine-grained memory
sharing.
\rb{Introduce our name for these traces here or later?}
%% \rb{This is our starting point and the bases of this work. Our goal is to
%% generalize this to fine-grained memory sharing.}

%% Still in this original setting, component memories are completely watertight and
%% the only means of communication between components is through the passing of
%% call arguments and return values. which cannot be pointers.

The deceivingly simple addition of pointer passing to procedure calls and
returns, a trivial change in both language semantics, results in a much more
expressive setting with deep implications for the proof of secure compilation.
While the compiler itself is unchanged and the top-level structure of
the \rscdcmd proof technique will survive with a few conceptual changes, its
parts must undergo very significant modifications. These adaptations, summarized
here, affect for the most part those proof obligations that are specific to the
proof technique, namely back-translation and recombination.

%% relatively small/local conceptual changes

%% can be adapted/survives the transition to the trace-relating
%% scenario with relatively few high-level changes, its constituents undergo very

\rb{TODO: Note advantage of proof reuse (here or immediately after?). Also that
blame is not really affected by the changes.}

\rb{Mention full\ch{?} mechanization of this too, amenability to modifications, etc.}

\rb{TODO: Mark changes in diagram, adjust notation.}

%% \subsubsection{Key Adaptations}

%% \subsubsection{Changes to the Languages}
\subsubsection{Surface Changes}

\ch{The main change with respect to CCS'18 is moving from an unsafe source
  language with a compiler that can refine undefined behavior, to a safe
  language in which there is no undefined behavior, and stuckness is preserved
  because of enforcement in the target. This is a change in the correct
  compilation statement (both FCC that can now take all traces and BCC that
  no longer produces a disjunction).}

%% Our technique is adapted from the original proof technique of \rscdcmd
%% \cite{AbateABEFHLPST18}. This technique was developed to

\rb{Briefly explain what pointers are (component, block, offset) and the
extension with a code/data permission bit. Note also that block identifiers are
abstract and unforgeable, and that they can be seen as a form of capability.}

Both source and target languages are generalized to allow the passing of pointer
values in calls and returns. This change leads to a refinement of certain
aspects of program well-formedness, in particular regarding where to allow the
presence of hardcoded pointer values in the programs and their initial memory
contents, and where those may point to.


One of the advantages of this technique\ch{what technique?}
is that it reuses standard compiler correctness results,
can lower the burden of securing verified compilation chains\ldots
No changes to the compiler (there is sufficient enforcement), therefore no
changes to those proofs\ch{what proofs? FCC and BCC?}
Of course once a memory address is shared there is nothing we can do to protect it from modification without further changes to the semantics and therefore the protection mechanism (interestingly those would not change the compiler much)

\rb{Instances of the proof technique, explain what is ``easy about it''
FCC, BCC ``for granted'', ``standard''\ldots}

buffers as capabilities of sort


Trace-relating robustly safe compilation \cite{difftraces-esop}
\ch{Right, since now the pointers appear in the traces.}

\subsubsection{Changes to Trace Events}

The base trace model of \cite{AbateABEFHLPST18} records calls and returns: source and target
components, called procedures, and passed arguments and return values.

To begin with, it is not enough to retain the basic trace model of
\cite{AbateABEFHLPST18}, where \ldots. Other changes below as new events are added. \rb{Name this trace
model here?}

Add memories, as representations of sequence of changes occurred while in control (without order\ldots)

\rb{Language changes?}

\subsubsection{Introduction of the Trace Relation}
\label{sssec:key-changes-rel}

is too restrictive

The design of a suitable trace relation \ldots

Traces pointwise related

\subsubsection{Changes to Back-Translation}
\label{sssec:key-changes-backtr}

\ch{If I remember right, at a high level the way the back-translation function
  works doesn't change much, but the invariants in the proof get much more complicated.}

%% back-translation as ``event replay''

\rb{Connect with references to the main proof, as with recomposition below?}

The original back-translation process is fairly simple. Take a finite trace \com{m} of
cross-component calls and returns, which we will call {\noninftraceTerm}s.
\rb{Introduce here or later?}
Take also an interface \com{I} is assumed to be the interface of the program
that produced \com{m}. \com{I} defines the set of compartments and the set of
exported procedures for each compartment and, because \com{m} was produced by a
program with interface \com{I}, each event in \com{m} can be assigned to one of
the procedures exported by \com{I}.

Therefore, the behavior of a compartment (resp. each of its exported procedures)
is defined by the projection of the trace on the events originating in that
compartment (resp., each compartment and procedure).
%
Each procedure subtrace is encoded as an expression in the source (i.e., the
body of the back-translated procedure) that simply replays the sequence of
events as calls and returns whose destinations and passed values are the
constants hardwired in the trace. Each component keeps track of the state of
the execution through an \rb{(local?)} event counter.
\rb{Place for an example here?}

The proof that this back-translation function satisfies the corresponding
assumption\ch{what assumption?}
of \rscdcmd \rb{(add reference)} is more interesting. To show that
the source output produces \com{m}, the main {\em definability lemma} proceeds
by a subtle induction on suffixes of \com{m}, showing that for any
partition \com{m = p \cdot s} and any program state consistent with the
execution of the prefix \com{p} (i.e., the simulation invariant), the execution
continues to completion and produces the rest of the trace \com{s}.
\rb{I wonder if this, and the paragraph that follows, get into too much detail.}
\ch{yes they do, it was supposed to be a ``key ideas'' section, not
  an ``all ideas'' one}

Establishing horizontal compositionality at the level of
compartments is easy, given that traces can be cleanly segmented \rb{better
word?} and contain all the information required to reproduce the story of
interactions.
%
The code of the back-translation can be decomposed into a sequence of code
blocks, each simulating a single event, so proving the inductive step reduces to
a case analysis on events, relating the contents of the memory after
simulating \com{p} to the matching code block for the next event in \com{s}.
Reestablishing the invariant after executing the steps in the code block is
simple, because metadata manipulation is limited to the local replay counter.

\rb{This will sound very similar to what I wrote below for recombination, so I
may want to make some generic comments about these parts and proceed to the
summary of important changes.}

\begin{itemize}

\item In keeping with the trace-relating setting, the back-translated \CsPprime
needs to produce not necessarily \com{m} itself, but a trace related to it, as
is indeed the case. This is because back-translated components employ a
private metadata buffer \rb{, not present in the original components}, on top of which programs may allocate additional
``public'' (i.e., shareable) buffers. According to the shifting scheme of the
trace relation, the back-translation will reserve the first buffer for its metadata,
and other buffers will reflect those of the \com{m} {\em offset by one}.
\rb{This last part needs to be clearer/more graphical.}

\item
The critical observation is that {\noninftraceTerm}s no longer provide enough
information to replay the execution, not least because passed values may depend
on individual memories, whose contents will be related but possibly different.
We need to move to a much more informative trace model to keep track of all
target operations that could have an effect on memory contents (\rb{examples});
we call these {\em {\inftraceTerm}s}. The back-translation
assumption \rb{(ref?)} needs to be rephrased in term of this new trace model.
\rb{Maybe give short notations to the two types of traces, like B- and S-traces?}

\item
The introduction of {\inftraceTerm}s requires the enrichment of the target
semantics and the addition of projection operations going from {\inftraceTerm}s
(and their executions) to the old {\noninftraceTerm}s. These projections
percolate the statements of the top-level theorem and its assumptions to
connect the informative semantics required by back-translation, which is only
meaningful at the target level, with the simpler interaction model that remains
the shared language between source and target.

%% ; trace projections all over the proofs, statements
%% ;  wrapping of target semantics, two; not so source (maybe talk about wrapping later)
%% ; relational rephrasing
%% ; explain connection to trace relation, metadata

\item
Internally, the simulation strategy of the back-translation function needs to be
altered to closely replicate a target execution in the source language. It does
so by simulating the register file of the abstract machine in the compartments'
metadata buffer, replaying all operations on registers in that memory. Call and
return events no longer pass concrete values hardcoded in the trace, and instead
need to reproduce the calling convention of the target, also in the source.
However, the general strategy of event counting remains unchanged.
\rb{Need to outline the increased payload of more informative traces (references
to registers, register contents) above, without becoming muddled.}

\item As a consequence of the above considerations, the back-translation
function needs a to take a new parameter: the initial memory contents of the
program that generated the trace \com{m}. Before starting the event replay, an
output source compartment must initialize its memory the contents of the
corresponding input source compartment, as these have an influence on the
simulated target execution. After that point, the source and target memories are
related by the shifting relation. \rb{Make sure this one is mentioned above.}
\rb{This forces some changes and clarifications also at the level of language
definitions, but is probably too much to mention here.}

%% ; Before we needed very little metadata, now a little more, but not much,
%% replicate register file, simulate execution in abstract machine

\item All these changes require us to maintain much richer memory invariants
relating the contents of the memories and the register files (real and
simulated), and synchronizing the contents of the memories with those of the
metadata buffer at certain events.
\rb{What else to say about this?}

%% before, relatively simple invariants

\end{itemize}

\rb{There is a general point to be made, here as elsewhere (notably in
recombination), that the general proof structure can be retained at a certain
level of abstraction, while stressing that the proofs themselves become harder
(and longer).}\ch{right, it would be good to make this point before getting
  into a sea of details.}

\subsubsection{Changes to Recombination}
\label{sssec:key-changes-recomp}

The original proof of recombination is a three-way simulation that takes two
pairs of programs and contexts \CtPcomp and \CscompPprimecomp, each producing
the same trace prefix \com{m}, and infers the existence of a third, equivalent
execution on \CscompPcomp. The gist of that proof is an induction on \com{m}
that reproduces the execution of \com{m} in the derived \CscompPcomp by
mimicking the steps taken by the two assumed runs.

Each of the two runs of \CtPcomp and \CscompPprimecomp consists of a series of
execution steps. The two runs synchronize whenever an observable event takes
place and produces the same interaction on both. Between synchronization points,
each of the runs may execute an arbitrary number of silent steps. Irrespective
of this, \rb{we know that} all silent steps between events are either in the
programs \Pcomp and \Pprimecomp, or in the contexts \Ct and \Cscomp.
%
Therefore, the derived run of \CscompPcomp simply takes the same steps
as \CtPcomp whenever the programs are running, and the same steps
as \CscompPprimecomp whenever the contexts are running.
%
\rb{(Above, we also know that steps that they are in the same component and that
component changes are replicated.)}
%
\rb{\ldots To be easily understandable, we may need to say something about
CompCert-style simulations. Lockstep may also be mentioned here. Try to avoid
too many details as much as possible. Probably a figure?}\ch{+1}

The correctness and relative simplicity of the above argument crucially relies
on the watertight sealing of compartments. Thanks to this property, the state of
the machine during execution can be cleanly composed as a union of independent
{\em compartment sub-states}. While a compartment is executing, it can only
modify its local state, leaving all others unaltered. This makes it easy to
write a function that {\em merges} the states of the two reference runs
piecewise into the state of the third derived run.

%% A program state is the union of the individual component states. In the absence
%% of memory sharing, there can be no interference between these component states.
%% That is, the currently executing component can only modify its own local state
%% while it maintains control; all other parts of the state remain unaltered. For
%% this reason it is simple to write a function that combines the current states of
%% \CtPcomp and \CscompPprimecomp piecewise into the corresponding state of
%% \CscompPcomp. When components can share parts of their memories by pointer
%% passing, this simple treatment no longer suffices.

In the presence of memory sharing, these simple properties of noninterference
and composability disappear. In moving to the relational setting, the general
structure of the simulation can be preserved, but the proof and its setup
undergo deep modifications, the most salient of which are sketched now.
\rb{Nexus to what's coming? Anything else? (Also, more inlined? Give them
names or references?)}

\begin{itemize}

\item
To begin with, the two whole programs \CtPcomp and \CscompPprimecomp now produce
related but different traces (prefixes, to be precise), and the derived run
of \CscompPcomp must similarly produce a third trace, itself related to its
forebears. While the trace relation preserves the synchronicity of events and
control transfers, the values passed back and forth may differ, as the contents
of the memories of \Pcomp and \Pprimecomp, on the one hand, and \Ct and \Cscomp,
on the other, are not identical, {\em even though they are related}.

\item
The simulation invariants and their use throughout the proof must be completely
redesigned. Whereas the original invariants related pairs of input states
from \CtPcomp and \CscompPprimecomp, and used a state merging function to
obtain the corresponding output state from \CscompPcomp, it becomes necessary to {\em relate
state triples} from all three programs, incorporating the steps of \CscompPcomp as
they are derived.

\item
The content of the invariants themselves becomes richer. In addition to the
trace relation, a {\em memory relation} and a {\em register relation} come into
play to keep track of related values as they flow through the executions.
\rb{What else to say here? Probably how and which parts of the memory are
related, for reference in the point about strong and weak relation.}

\item
In place of the old binary invariant that is preserved at each step of the
simulation, the required {\em ternary invariant} is actually the composition of {\em two
binary invariants}, relating the output run of \CscompPcomp with each of the
input runs of \CtPcomp and \CscompPprimecomp. Each of these sub-invariants is
active according to which parts are currently executing: when the programs are
running, the states of \CtPcomp and \CscompPcomp are pairwise related; when the
contexts are running, it is the states of \CscompPprimecomp and \CscompPcomp
that are related in turn.

\item
The memory \rb{sic?} relation is actually divided into two: a {\em weak
relation} which must hold at all steps during the simulation, and a {\em strong
relation} which holds immediately after a call or a return.
\rb{Complete this a bit more, give an intuition, strengthening and weakening.
An example would probably be quite good here. Synchronization between binary
invariants.}

\end{itemize}

\rb{Formulate this with math here? Do it later?}
\rb{I wonder if one should make more references to concepts of renaming and so
on, described above, or keep it abstract}
\rb{Possible use of examples, comparisons, etc.}
\ldots

\paragraph{Other Changes}

Small simplifications? Blame. Extended well-formedness conditions, mostly to
clarify pointer provenance. Not simplifications as much as precisions.

\begin{itemize}

\item Basic program and trace model \rb{It may be misleading to describe traces
and ``non-informative'' vs. ``informative''. One trace model has more
information than the other, though maybe more descriptive names could work and
be introduced gradually.}

      \begin{itemize}

      \item Compartments

      \item Interfaces and procedures

      \item ``Noninformative'' events

      \end{itemize}

\item Basic proof overview

\item Memory sharing model

\item Trace relations

\item Security property

\item Example/running examples

\item Mechanization

\end{itemize}

\rb{I think the word ``original'' is repeating too much. Maybe use \rscdcmd as
qualifier? The IEEE style of citation doesn't make inline references to the paper
very nice.}

\ifdraft
\clearpage
\fi

\section{Technical Framework}

\ldots

\input{source-syntax}

\input{target-syntax}

Syntax in \autoref{fig:source-syntax} and \autoref{fig:target-syntax}

\rb{memory model, CompCert style, adjustments and reliance on
certain behaviors (allocator, etc.) to simplify proofs; unforgeable pointers}

\rb{compartmentalizing secure compilation}

\section{A Trace Relation for Memory Sharing}

Each component declares a set of private blocks that will never be shared with
other components. \rb{Blocks are abstract and unforgeable, so we can assume
w.l.o.g. that these are the first few natural numbers to make things more
concrete. Later, when we manipulate back-translated programs, those private
blocks will represent the blocks that contain metadata used to simulate trace
behavior.}

Shifting as a special form of renaming.

\aek{When presenting definitions and lemmas for
memory renaming, we should try to draw connections
to the work of
\cite{zhirkov2019memory} (which I just came across now)
on memory bijections for reasoning
about refactorings in CompCert C.}

Each component may or may not have a number blocks that will of metadata blocks
at the front. These must never be shared.

Renaming will be applied to traces as well, given that addresses will appear on
traces.

\section{\titlecap{\inftraceTerm} Back-Translation}

\subsection{Generalities}

The proof of \rb{criterion} involves the back-translation of an
arbitrary \rb{(``informative'')} finite trace prefix \finprefInf produced by the
whole target program \CtPcomp into a source program $\back{(\CtPcomp)}$ which
produces an ``equivalent'' version of the same trace. \rb{How are the traces
related? First, the source language does not have ``informative'' events, so the
back-translated trace must be projected to its ``non-informative'' fragment.
Second, renaming must be taken into account, but we need to explain the
back-translation for that.}

More precisely, the back-translation function takes a finite \rb{informative}
trace \finprefInf and the whole (target) \emph{program} that produced it as
inputs. \rb{This is no longer just the interface due to the need to
back-translate static buffers, cf. below, although we probably will not use
those explicitly in this presentation.} It produces a whole source program with
the same interface, and therefore the same components and exported procedures,
where the code of each (exported) procedure is back-translated
independently. \rb{Define each part of the output separately? Interface,
buffers, procedures. Better, and/or first, give an idea of how the program is
supposed to behave, refer to example.}

\ldots

Each source component declares statically a local buffer and may allocate
additional buffers dynamically. A back-translated component uses its local
buffer for bookkeeping of back-translation metadata, in a manner that will be
described presently.

A target component may define an arbitrary number of static buffers. If it does
so, its corresponding back-translated source component needs to be prefixed by
an initialization step. Namely, before the component starts
simulating \rb{target, informative} trace events, it needs to execute code to
allocate as many static buffers as defined by the original target component, and
initialize them with the static contents of the buffers as given by the program
definition. \rb{Note that to preserve the constant offset that we use in the
relation, this relies on a predictable allocator of new blocks, the details of
which will normally be hidden from the user. In addition to this, the static
contents of the buffers may not contain pointer values, otherwise more
sophisticated mechanisms are required.} \rb{For simplicity of exposition, we
consider here the simplified case where back-translated target components do not
define any static buffers, using code instead to declare and initialize those.}

\ldots

Each procedure is back-translated as follows. \ldots

\ldots

Because our back-translation technique is compositional on program components,
we can split the back-translated whole program by provenance into the
back-translation of the original compiled program, $\back{(\Pcomp)}$, and the
back-translation of the context, $\back{\Ct} = \Cs$, which we will take as our
source context in subsequent stages of the proof.

\rb{The back-translation does not use the program, only its interface -- and
later its buffers will be added.}

\subsection{Adaptations}

\begin{itemize}

\item Moving to a very informative trace model, which exposes many of the
details of the execution of a target program.

\item The basic mechanism to replicate the execution remains essentially
unchanged.

\item How do the more informative traces simplify the back-translation? How
does it connect to the rest of the proof?

\item Compare e.g. to the ample amounts of metadata required by the CapablePtrs
back-translation. Here we are much closer to ``lockstep'' and the metadata that
we require is little and simple, with few additions. \rb{Point of illustration:
find an example and compare the two. Simple lockstep simulation vs. much harder
alternative \ldots. (In fact, PC lockstep.)}

\item Tradeoffs: this setup would not work for unsafe languages. If there is
anything in the target language that is hard to reproduce in the source
language.

\item Richer memory invariants

\item Explain rich traces here: registers (provenance), values of the registers
(values must be related), etc. Later, at the border, we will need this
information to restore the strong memory relation. \rb{Getting ahead of
ourselves? We need it for the stepwise memory invariants too.}

\item Syntactically, the generated back-translation and the code generation
strategy are similar. Proofs become substantially more complex, though the
general structure is preserved.

\end{itemize}

\rb{Vantage points: we get a simple(r) back-translation by looking at the whole
program. And we look at the program created by back-translation, which
simplifies things -- as look as we keep the program/context divide intact.}

\rb{May want to say something about internal calls and why we don't need to care
about them}
\rb{General setup, interesting bits, well-bracketedness?}

\section{Relational Recomposition}

\subsection{Generalities}

Recomposition is a proof technique developed to subsume and simplify the proofs
of decomposition and composition employed by the original proof of \rscdcmd
in \cite{AbateABEFHLPST18}. In its basic form, it considers a whole program interface,
arbitrarily split into a ``program'' part and a ``context'' part, and two whole
programs that conform to this interface, say, \PaCa and \PbCb. The recomposition
theorem states that if both whole programs produce the same finite
trace \finpref, then we can swap the program and context parts to produce,
say, \PaCb, another whole program that also produces the finite trace \finpref.

\rb{In the proof of \rscdcmd, recomposition is proved for the target
(``intermediate'') language with standard ``non-informative'' (call-return)
traces. This model is preserved in the new relational proof with memory
sharing.}

\rb{Outline}

Symmetry, case analysis on which part of the program, ``program'' side or
``context'' side, starts the execution, based on where the main procedure lives.

\rb{From above: organization of the proof becomes slightly less modular (put
together invariants and steps, etc.)}
\rb{Maybe mention in overview? The new trace and the obligation of relatedness,
etc., there are additional top-level proof obligations, though these are as
expected}
\rb{Towards a more intensional proof of recomposition, invariants, etc. (Anything
to hint at the top?)}

\subsection{Relational Extensions}

\rb{Adaptations}

What is the effect of memory sharing on the general technique?

Generalized technique.

Instead of relating ``compatible'' pairs of states \Saa and \Sbb and relying on
a ``merging function'' that can derive the corresponding state from the combined
run, we add this third state explicitly \Sab. The ternary relation is defined in
terms of a binary relation between states (and \ldots), which relates the
``third state'' in the combined run to one of the other states, depending on
which part, program or context, controls the execution at the moment. If the
program parts are running, \strel{\Saa} is used; and if the context parts are
running, \strel{\Sbb} is used to relate the combined state and the state on
which the relation is defined. \rb{This needs exposition work, of course. We
don't neglect the ``unrelated part,'' though we do instantiate one relation in
two different ways.}

Strong and weak relations. Simulation relation.

\begin{itemize}

\item The strong relation holds immediately after a cross-component call or
return.

\item The weak relation holds at all times.

\item A simple weakening lemma can always be used to derive the weak relation
from the strong one.

\item Strengthening must be used to reestablish the strong relation at boundary
crossings. \rb{Is this actually phrased as a ``current component vs. all
others'' as opposed to a ``program vs. context'' property?}

\end{itemize}

Distinction between border states and internal states. \rb{This distinction
could be implicit, and closer to the non-relational proof, but more case
analysis would be needed. Harder? Akram thinks so.}

\begin{itemize}

\item Need for a relation: adequacy, connection to top-level result, which
concerns the trace relation, which talks about relatedness of shared addresses,
i.e., the contents of the memories at those shared addresses \rb{related, not
necessarily the same on both sides}.

\item However, while executing within a component the relation between the
contents of the memories may not hold (i.e., does not need to hold at all times;
it may be temporarily violated and restored later).

\item At the border states, the contents of the memories of all three states are
related.

\item Relate parts of the memory actively executing (or reachable from there)
and those that are not \rb{remain unchanged}.

\item Internal states: relate memory parts that are not executing. First exclude
shared addresses, as those may be changed by the executing part. That is,
consider all the private memory of the combined program. E.g., when
relating \Saa and \Sab (execution in \Pa), we remove all the private and shared
state of \Pa, i.e., we (can) only relate the private state of \Cb. Later on, we
may switch sides and therefore need to say that the whole reachable memory
of \Pb is related.

\end{itemize}

Statement \rb{only for compiled programs -- for us, compiled, more general
lemmas would be possible -- see below}

Instantiation in the overall proof diagram \ldots

\rb{The strong and weak relations are another point of ``comparison'' with
CapablePtrs, which conceptually require a very similar setup -- however that
work is targeting full abstraction, however there is no recombination there.
This is inherently about triplets of programs. CapablePtrs also had triplets,
and some similarities arise. Does recombination by itself already simplify
things substantially relative to CapablePtrs? Ends up being simpler overall.}

\rb{One difference: we are relating three target programs vs. a combination
of source and target programs in CapablePtrs. We stay at the same level.
In that sense at least it is a simplification of sorts (we compile the full
back-translation and recombine with that). Recombination also does not say
anything at all about the compiler.}

\rb{The compiler isn't doing anything interesting w.r.t. security. This may be
why we can reduce some things to compiler correctness and then disregard the
compiler otherwise. E.g., SFI would break things. CapablePtrs only looks at
compiled programs.}

\rb{Freedom of how to back-translate the program.}

\rb{Trace projections on levels of detail as novelty. Novelty of very
informative traces, lockstep back-translation w.r.t. lower level.}

\rb{Going lower in enforcement, backends, micropolicies, etc.}

\subsection{Discussion}

\rb{Example to show why recomposition with shared memory is much harder.
Akram had ideas about this, according to Deepak? Private memory on both
sides to motivate the two relations.}

\ifdraft
\clearpage
\fi

\section{Related Work}

CapablePtrs \cite{} \ldots \rb{Proof technique for full abstraction in the
pointers-as-capabilities model, more than a generic proof technique?}

Multiple traces

Compositional compilation, esp. CompComp, also re: reachability relations, etc.

\rb{Any other secure compilers w.r.t. interesting trace relations like this
one?}

\section{Conclusion}

\begin{itemize}

\item The ``lockstep''/``synchronous'' back-translation should make it
relatively simply to adapt to the concurrent case.

\item Proving stronger criteria, effects notably on back-translation and the
need to back-translate several traces simultaneously. Pointwise lifting, small
and local impact expected on the proof.

\item Trade-offs of the informative model: other features facilitated or
complicated by it.

\item Is this where we discuss the mechanization?

\item We probably need to discuss full abstraction at some point and motivate
our choice of a different criterion.

\item Other potential instances of the proof, going lower\ldots

\end{itemize}


==> proof-diagram-old.tex <==
% !TEX root = ./paper.tex

\begin{tikzpicture}[auto]
\node(cPi) {$(\trg{C_t}\ \trg{\cup}\ \cmp{\src{P}})\  \trg{\doesprefix}\ t_1$ };
\node[right = of cPi] (CP1t) { $(\cmp{\src{C_s}}\ \src{\cup}\ \cmp{\src{P'}})\ \trg{\doesprefix}\ t_2$ };
\node[align = left, above = of cPi] (CP1s) { $\back{t_1\ }$ $= (\src{C_s}\ \src{\cup}\ \src{P'})\  \src{\doesprefix}\ t_\mi{backtr}$ };
\node[right = of CP1t, xshift=2em] (CPt) { $(\cmp{\src{C_s}}\ \src{\cup}\ \cmp{\src{P}})\  \trg{\doesprefix}\ t_{1,2}$ };
%  \node[above = of cPi, xshift=12em, yshift=1.5em] (prec) { $m \leq t \lor t \prec_P m$ };
\node[above = of CPt] (CPs) { $(\src{C_s}\ \src{\cup}\ \src{P})\ \src{\doesprefix}\ t_{\mi{QED}} %\wedge (m \leq t \lor t \prec m)
	$
};


\draw[->] (cPi.90) to node {\hyperref[lemma-abateetal-backtrans]{\em 1 Back-translation}} (CP1s.-90);

\draw[->] (CP1s.-45) to node [align=left,font=\itshape,xshift=-0.25em,yshift=-0.3em]{\hyperref[assm-fwdsim]{2 Forward Compiler Correctness}} (CP1t.180);

%\draw[->] (CP1s.-8) to node [right,yshift=-0.5em, xshift=3em]{\em \hyperref[asm:blame]{5 Blame}} (prec.180);
%\draw[->] (CPs.140) to node {} (prec.0);

% composition target
\draw[->] (CP1t.0) to node [below,xshift=0em,yshift=-0.5em]{\em \hyperref[lemma-abateetal-recomb]{3 Recomposition}} (CPt.180);
\coordinate [below=1.5em of CP1t,xshift=0em] (compoint1);
\coordinate [below=1.5em of CPt,xshift=-4em] (compoint2);
\draw[-] (cPi) to (compoint1);
\draw[-] (compoint1) to (compoint2);
\draw[->] (compoint2) to (CPt.220);

\draw[->] (CPt.90) to node [right,align=left,font=\itshape]{\hyperref[assm-bwdsim]{4 Backward Compiler Correctness}} (CPs.-90);

% side labels
\node[left = of CP1s, xshift=0em] () {\color{gray} Source};
\node[left = of cPi, xshift=-1.5em,yshift=0.2em] () {\color{gray} Target};
\end{tikzpicture}


==> robustptrs.tex <==
% !TEX root = ./paper.tex

In \robustptrs, we plan to prove a different compiler
 security property, namely, robust preservation of 
 safety. This time, I am verifying the proof 
 mechanically in Coq. This is the first mechanized 
 proof of this
property
for languages that allow memory sharing through
pointer passing.
The only other mechanized proof of this property
that we are aware of is the one by 
\citet{Abate:2018:GCG:3243734.3243745}, in which 
the languages do not allow any means for memory
sharing between program components.

\subsection{Source and Target Languages}

%Our source language is
%an imperative C-like expression language (that I will
%call \sourcelanguageShare), and our target
%is a compiler intermediate
%language with instructions and registers
%(that I will call \intermediatelanguage).
%Compared to \targetlanguage of \capableptrs, 
%\intermediatelanguage is a more realistic intermediate
%language that features only instructions and registers
%(rather than expressions as in \targetlanguage),
%but the key similarity is that \intermediatelanguage
%(just like \targetlanguage) features a separate
%run-time type for \emph{unforgeable
%pointers} that carry bounds and permissions 
%(hence, modeling capabilities)\footnote{
%	Going forward, in \Cref{sec:robustptrs}, the use of
%	\src{this\ blue\ font} is reserved for 
%	\sourcelanguageShare elements, and the use of
%	\trg{this\ red\ font} is reserved for
%	\intermediatelanguage elements.}.
%
%The semantics of both \sourcelanguageShare
%and \intermediatelanguage are built on top of a 
%CompCert-like
%memory model, and the languages are inspired by the 
%prior work
%by \citet{Abate:2018:GCG:3243734.3243745}, but with
%two key differences: (1) Pointers in both
%\sourcelanguageShare and \intermediatelanguage
%carry more 
%information (than the pointers of
%\cite{Abate:2018:GCG:3243734.3243745}), 
%namely, an extra permissions field, and
%(2) Both \sourcelanguageShare and
%\intermediatelanguage (unlike in
% \cite{Abate:2018:GCG:3243734.3243745})
%support passing pointers across module boundaries.
%Allowing pointer passing across module boundaries is
%the key technical challenge that \robustptrs tackles.


%The semantics
%of both \sourcelanguageNoshare and 
%\intermediatelanguageNoShare
%prohibit (at run time) 
%passing pointers across module boundaries
%(think of a module as a C compilation unit), a 
%prohibition that limits the nature of interaction
%between a program part
%and a third-party library;
%a third-party library is typically provided either as 
%a separate module/compilation unit. Thus,
%the prohibition on passing pointers meant that basic
%data structures could not be passed as arguments
%to such library.
%Instead, to copy/share a data structure,
%the data structure
%would have to be rebuilt through successive
%API calls (to the library) that would 
%insert one base value per call, which
%is clearly unrealistic because it lacks convenience and
%runtime efficiency.

%We lift this prohibition on passing pointers, which
%results in a pair of languages that, despite remaining
%syntactically similar to \sourcelanguageNoshare and
%\intermediatelanguageNoShare, are now a more
%faithful (although still simplified)
%model of C (\sourcelanguageShare) and of 
%an intermediate language of a C compiler 
%(\intermediatelanguage). Lifting this prohibition
%results in a non-trivial ripple effect throughout
%the proof as we explain in \Cref{sec:recombination}
%below. 
%
%Before getting there, we show below the syntax of both
%\sourcelanguageShare and \intermediatelanguage, which
%is still very similar to the syntax (given in 
%\cite{Abate:2018:GCG:3243734.3243745}) of their
%predecessor pair of languages. The
%only difference in syntax is our addition of
%a \trg{PtrOfLabel} instruction in 
%\intermediatelanguage, which did not exist in
%\intermediatelanguageNoShare.
%We need this instruction to be able to compile function
%pointers, a newly added feature of the source.
%\todo[inline]{add function pointers to the source syntax}
%\begin{align*}
%\src{e}  ::=\  
%        & \src{v}               &\text{values}
%\\\mid\ & \src{local}           &\text{fixed name of the local buffer}
%\\\mid\ & \src{e_1 \otimes e_2} &\text{binary operations}
%\\\mid\ & \src{e_1; e_2}        &\text{sequence}
%\\\mid\ & \src{if\ e_1\ then\ e_2\ else\ e_3} &\text{conditional}
%\\\mid\ & \src{alloc\ e}         &\text{memory allocation}
%\\\mid\ & \src{^{*}e}            &\text{dereferencing}
%\\\mid\ & \src{e_1\ :=\ e_2}     &\text{assignment}
%\\\mid\ & \src{C.P(e)}           &\text{call to procedure \src{P}}
%\\\     &\                       &\text{of component \src{C} with argument \src{e}}
%\\\mid\ & \src{exit}             &\text{terminate}
%\end{align*}
%
%\begin{align*}
%\trg{instr}  ::=\  
%        & \trg{Nop}        & \mid\ \trg{Halt}
%\\\mid\ & \trg{Jal\ l}     & \mid\ \trg{Const\ i\ reg}
%\end{align*}
%......

As in \capableptrs, the semantics of both 
languages are aware of the concept of
a program component. Calls and returns that cross
a component boundary (i.e., a call/return to a 
function defined by a component that is 
different from the 
component defining the currently executing function)
show up on the trace as an observable event.
On the other hand, calls and returns to the currently 
executing component
do not show up as an observable event. With this
definition of an observable event in hand, we write
$P \rightsquigarrow^{*} m$ to denote that a whole 
program $P$ emits an observable trace prefix $m$.


\subsection{The Compiler Security Criterion: Robust Preservation of Safety}

A safety property is a property that can be specified
as a set of bad prefixes. To prove that the compiler
robustly preserves all safety properties of source
programs, it suffices~\cite{abate2019journey} to prove point-wise that any (bad) 
prefix $m$ emitted by a compiled program 
$\src{P}\downarrow$ in some target context \trg{C}
can be attributed to a related bad prefix $\tilde{m}$
that the source program \src{P} emitted in
some source context \src{C}. More formally, we would
like to prove (for some sensible choice of a 
trace relation $\sim$) the following statement:
%\begin{definition}[Compiler $\downarrow$ robustly
%	preserves safety]\label{rsp-def}
%\begin{align*}
%&\textbf{RSP}(\downarrow)~\defeq\\
%&\forall \src{P}\ \trg{C}\ m.\\
%&\trg{(C\ \cup\ }\src{P}\downarrow\trg{)}\ 
%\trg{\rightsquigarrow^{*}}\ m \implies
%\exists \src{C}\ \tilde{m}.~
%\src{(C \cup P)\ \rightsquigarrow^{*}}\ \tilde{m}\ 
%\wedge\ \tilde{m}\sim m
%\end{align*}
%\end{definition}

\subsubsection*{Choosing the trace relation $\sim$}

First of all, recall the use of traces in \capableptrs.
In \capableptrs, traces were used just as an
auxiliary tool for the purposes of the proof. They
did \emph{not} appear in the statement
of the top-level theorem
 (\Cref{theorem-full-abstraction} -- Full abstraction).
Moreover, the way we structured the proofs
required us to choose two relations
(an equivalence on sets of traces of source programs
and a similar equivalence on sets of target
traces) that were respectively constrained by
a soundness (\Cref{soundness-target-trace-equivalence}) and a completeness
 (\Cref{completeness-source-trace-equivalence}) lemma.

In contrast to the role of traces in \capableptrs,
here in \Cref{rsp-def}, traces and a trace
relation \emph{do appear} in the statement of the
top-level theorem. Thus, the choice of traces and
a trace relation is less constrained, and
one has to be careful which 
trace relation $\sim$ is chosen in the definition
of \textit{\textbf{RSP}}. Choosing a trace relation
that is too small might, e.g., lead to the detrimental
effect of excluding certain compiler
optimizations. Also, choosing a trace relation that
is too big might mean that the theorem is trivial
or not very meaningful because it requires too
little:
a given target trace prefix $m$ that is considered bad
will get away by finding a related (i.e., a justifying) 
source trace prefix $\tilde{m}$ even if
the compiler did not enforce any memory isolation
between components.

Moreover, the choice of the trace relation
is (as in \capableptrs and unlike in other prior
work \cite{Abate:2018:GCG:3243734.3243745}) 
affected by allowing memory sharing:
 Because in both the source and target languages, 
we still allow passing pointers across component
boundaries, a sensible choice of the trace relation
$\sim$ had better account for the parts of the
memory that become incrementally
shared (at run-time) through the
passing of pointers among components. 
We choose a trace relation $\sim$ such that this shared
memory is part of the observable behavior (trace) of
a program part (just like in the traces we chose
in \capableptrs), which effectively means that we allow 
specifying safety
properties on these shared parts of the memory.
More concretely, 
we choose a trace relation $\sim$ that ensures that
the \emph{memory shared so far} along the given
target execution $m$ is related to the \emph{memory
shared so far} along the justifying execution
$\tilde{m}$ of the source program.
However, unlike in \capableptrs, we additionally
allow the justifying trace $\tilde{m}$
to rename the memory addresses (i.e., the pointer 
values) that appear on the given trace $m$.

These two features of the top-level trace relation
$\sim$ (namely, ensuring that the memory shared so far
is related and allowing renaming of memory addresses)
also manifest in all the other auxiliary trace relations
that we use in the statement of some key lemmas.
The key lemmas are given next in
 \Cref{sec:proof-plan-robustptrs}, and the trace
relations will be denoted by $\sim_\mi{compiler}$,
$\sim_\mi{recomb}$ and $\sim_\mi{backtr}$. All three
are very similar in structure and are similar
to the main relation $\sim$, and they basically only
differ in what address renaming function 
they specify. 

\subsubsection*{Undefined behavior}
Because the a source program part can get
stuck when interacting with a source
context (stuckness that results from our semantics
not fully defining some of the undefined behaviors of
C), we plan to only prove a weaker form of 
\Cref{rsp-def}, which accounts for the possibility
that the source program part runs into undefined
behavior. This weakening is standard in the literature
on both compiler correctness formal guarantees 
\cite{leroy2009formal} and compiler security formal
guarantees \cite{Abate:2018:GCG:3243734.3243745}.
In compiler security literature
\cite{Abate:2018:GCG:3243734.3243745}, this weakening
has been referred to as a ``blame'' result---blaming
the failure to justify a given (bad) target trace on
the source program part because it allowed itself to
run into undefined source-language territory.

\begin{definition}[Compiler $\downarrow$ robustly
	preserves safety or blames the source program part
	\src{P} for an $\texttt{\textit{Undef}}(\src{P})$ event]
	\label{rspb-def}
\begin{align*}
&\textbf{RSPB}(\downarrow)~\defeq\\
&\forall \src{P}\ \trg{C}\ m.\\
&\trg{(C\ \cup\ }\src{P}\downarrow\trg{)}\ 
\trg{\rightsquigarrow^{*}}\ m \implies\\
&\ \ \ \ (\\
&\ \ \ \ \ \ \ \
(\exists \src{C}\ \tilde{m}.~
\src{(C \cup P)\ \rightsquigarrow^{*}}\ \tilde{m}\ \wedge
\tilde{m}\sim m)\\
&\ \ \ \ \ \ \ \ \
\vee\\
&\ \ \ \ \ \ \ \
(\exists \src{C}\ \tilde{m}'\ m'.~\\
&\ \ \ \ \ \ \ \ \ \ 
m' \leqslant\ m\ \wedge\ 
\src{(C \cup P)\ \rightsquigarrow^{*}}\ \tilde{m}'.\texttt{Undef}(\src{P})\ \wedge\  
\tilde{m}'\sim m')\\
&\ \ \ \ )
\end{align*}
\end{definition}

\subsection{High-level Plan of the Proof}
\label{sec:proof-plan-robustptrs}

To prove \textbf{\textit{RSPB($\downarrow$)}} 
(\Cref{rspb-def}), we rely on the following key lemmas:

\begin{lemma}[Compiler forward simulation 
	(whole-program)]\label{lemma-robustptrs-fwdsim}
\begin{align*}
&\forall \src{P}\ m.\ 
\src{P}\ \src{\rightsquigarrow^{*}}\ m \implies
\exists \tilde{m}.\ 
\src{P}\downarrow\ \trg{\rightsquigarrow^{*}}\ \tilde{m}\ 
\wedge\ m \sim_\mi{compiler} \tilde{m} 
\end{align*}
\end{lemma}


\begin{lemma}[Compiler backward simulation 
	(whole-program)]\label{lemma-robustptrs-bwdsim}
\begin{align*}
&\forall \src{P}\ m.\ 
\src{P}\downarrow\ \trg{\rightsquigarrow^{*}}\ m 
\implies\\
&\ \ \ (\\
&\ \ \ \ \ \ (\exists \tilde{m}.\ \src{P}\ 
\src{\rightsquigarrow^{*}}\ \tilde{m}\ \wedge\ 
\tilde{m} \sim_\mi{compiler} m
)\\
&\ \ \ \ \ \ \vee\\
&\ \ \ \ \ \ (\exists \tilde{m}'\ m'.\\
&\ \ \ \ \ \ \ 
m' \leqslant\ m\ \wedge\ 
\src{P\ \rightsquigarrow^{*}}\ 
\tilde{m}'.\texttt{Undef}(\src{P})\ \wedge\  
\tilde{m}'\sim_\mi{compiler} m'
)\\
&\ \ \ )
\end{align*}
\end{lemma}

\begin{lemma}[Recombination of target-language
programs that emit related traces]
\label{lemma-robustptrs-recomb}
\begin{align*}
&\forall \trg{P}\ \trg{C}\ \trg{P'}\ \trg{C'}\ 
m\ m''.\\
&\ \ \trg{(P \cup C)\ \rightsquigarrow^{*}\ }m \implies\\
&\ \ \trg{(P' \cup C')\ \rightsquigarrow^{*}\ }m'' \implies\\
&\ \ m \sim_\mi{recomb} m'' \implies\\
&\exists m'.\ \trg{(P \cup C')\ \rightsquigarrow^{*}\ }
m'\ \wedge\ m' \sim_\mi{recomb} m
\end{align*}
\end{lemma}

\begin{lemma}[Whole-program back-translation of
	target-language observable traces]
\label{lemma-robustptrs-backtrans}
\begin{align*}
&\forall \trg{P}\ m.\ 
\trg{P\ \rightsquigarrow^{*}\ }m \implies
\exists \src{P}\ \tilde{m}.\ 
\src{P \rightsquigarrow^{*}\ }\tilde{m}\ \wedge\ 
\tilde{m} \sim_\mi{backtr} m
\end{align*}
\end{lemma}

By relying on
 \Cref{lemma-robustptrs-backtrans,lemma-robustptrs-bwdsim,lemma-robustptrs-fwdsim,lemma-robustptrs-recomb},
we plan to prove that our compiler 
satisfies \textbf{\textit{R}}obust
\textbf{\textit{S}}afety
\textbf{\textit{P}}reservation with
\textbf{\textit{B}}lame (\Cref{rspb-def}).
Here is a sketch of the proof:

\begin{enumerate}
\item By the assumption of 
\textbf{\textit{RSPB($\downarrow$)}} (\Cref{rspb-def}),
we know that the target program
$\trg{C\ \cup\ }\src{P}\downarrow$ emits a trace, so
we instantiate \Cref{lemma-robustptrs-backtrans} 
(the back-translation lemma)
to obtain a related trace (call it $m_\mi{backtr}$)
and a whole program (call it \src{P_\mi{backtr}}) that
emits it. There are other structural lemmas that
tell us that \src{P_\mi{backtr}} consists of two
program parts with the same interfaces as the given
\trg{C} and $\src{P}\downarrow$ program parts.

\item With this source program \src{P_\mi{backtr}}
and its execution in hand, we now instantiate 
\Cref{lemma-robustptrs-fwdsim} to obtain a
related execution
of $\src{P_\mi{backtr}}\downarrow$, which we will call
$m_\mi{backtr.comp}$.

\item Now we have two target executions from two bipartite
programs (namely, the program $\trg{C\ \cup\ }\src{P}\downarrow$
from our assumption, and the program $\src{P_\mi{backtr}}\downarrow$ that we
just obtained), so we instantiate
\Cref{lemma-robustptrs-recomb} to obtain a related
target execution $m_\mi{recomb}$ of a recombined program that
consists of a left part coming from 
$\src{P_\mi{backtr}}\downarrow$ and a right part
coming from $\trg{C\ \cup\ }\src{P}\downarrow$.
We will write this recombined program as
$\src{C_\mi{backtr}}\downarrow\ \trg{\cup}\ \src{P}\downarrow$.

\item By applying
structural lemmas about separate compilation,
we can now view this recombined program
 $\src{C_\mi{backtr}}\downarrow\ \trg{\cup}\ \src{P}\downarrow$ 
from the previous step as the
compilation of the whole source 
program \src{C_\mi{backtr}\ \cup\ P}. 
Viewing it as a whole-program compilation allows us to
instantiate \Cref{lemma-robustptrs-bwdsim} (whole-program
backward simulation) to finally obtain the conclusion
of \Cref{rspb-def}, which is our goal.
\end{enumerate}

Lots of the work so far has gone into proving
\Cref{lemma-robustptrs-recomb} (Recombination) and 
\Cref{lemma-robustptrs-backtrans} (Back-translation), 
both still work in progress (see \Cref{sec:timeline}).
Next, we discuss one novel technical contribution
for proving \Cref{lemma-robustptrs-backtrans}.

%\todo[inline]{START: Think of a story}
%
%The semantics of \sourcelanguageShare and
%\intermediatelanguage is based on a block-based
%memory model similar to the CompCert memory model.
%
%
%
%\subsubsection{Two approaches to back-translation in prior work}
%
%Techniques for back-translation from prior work (which is covered in
%the survey by
%\citet{Patrignani:2019:FAS:3303862.3280984})
%can be classified broadly into two
%approaches: \emph{syntax-directed} and \emph{trace-based} 
%back-translation. Syntax-directed back-translation 
%has seen a lot of development especially by the work of
%\citet{New} (multi-language semantics)
%and \citet{popl-backtrans,DBLP:journals/lmcs/DevriesePPK17} (approximate back-translation).
%Other syntax-directed back-translation techniques include
%the work by
%\citet{Skorstengaard:2019:SEW:3302515.3290332}\footnote{
%	More discussion of \citet{Skorstengaard:2019:SEW:3302515.3290332}
%	is in \Cref{sec:related-work}.}
%(a logical relation with recursive worlds).
%
%Trace-directed back-translation has been used to make security arguments
%about target languages that model low-level security primitives, e.g.,
%Protected Module Architectures
%\cite{agten,mfac,patrignani2015secure,marcothesis},
%tagged architectures \cite{Abate:2018:GCG:3243734.3243745,catalin},
%and enclaves \cite{busi2020provably}.
%In this paper, we take the trace-based back-translation approach
%to prove that compilation to capability machines is secure.
%
%By modeling a \pac compiler and proving that it is secure, we 
%are the first to show how the trace-based back-translation approach
%can scale to languages with fine-grained memory sharing.
%All prior work mentioned above that uses trace-based back-translation
%used to model languages where sharing memory between the program and
%the context (or across module boundaries in general) was prohibited.
%
%\subsubsection{Trace-based back-translation}
%\label{trace-based-backtrans-background}
%
%To understand the challenge in adapting the trace-based back-translation
%approach to fine-grained memory sharing, let us dig a bit deeper into
%the proof of condition \ref{condition-preserves}, then see how
%traces from prior work look like, and contrast this with
%traces in our model (that are imposed by fine-grained memory sharing).
%
%The reason why this proof step becomes considerably more challenging
%with fine-grained memory sharing is because the alphabet of
%the actions that appear on
%a trace $\alpha$ becomes more complex. (Notice that the choice
%of this alphabet is constrained by the soundness and completeness
%conditions of 
%\Cref{soundness-target-trace-equivalence,completeness-source-trace-equivalence}
%respectively.)
%
%In all prior work, 
%the alphabet of trace actions (or labels $\lambda$) 
%looks like this\footnote{The notation of $?$ and $!$ decorators
%	is inspired by process
%	calculi~\cite{milner1999communicating} and refers here
%	to the direction of the change of control (context to program of interest or vice versa).}:
%\begin{align*}
%\lambda_{\mi{prior\_work}} ::= ~\tau \mid \checkmark &\mid
%\mathtt{call}(\mi{fid}) ~?~\OB{v}
%\mid
%\mathtt{call}(\mi{fid}) ~!~\OB{v}
%\\
%&\mid
%\mathtt{ret}~?~v
%% \\
%% &
%\mid
%\mathtt{ret}~!~v
%\end{align*}
%
%Thus, without fine-grained memory sharing, 
%\emph{Hypothesis 2} gives a trace prefix $\alpha$ that is
%effectively a description of a 
%sequence of call and return actions, each call
%with call arguments, and each return with a return value.
%To solve the \textbf{goal} above, one had to find
%a context $\ctxs_{\src{emu}}$
%that will initiate the correct ?-decorated action
%every time it receives back control (through an !-decorated action).
%The arguments and the return values to be mimicked
%can be simply hard-coded in the code of
%the emulating context $\ctxs_{\src{emu}}$, and that is what all prior
%work does (see, e.g., figure 8 of \citet{Abate:2018:GCG:3243734.3243745}). 
%
%\setulcolor{red}
%Thus, in all prior work, the emulating context $\ctxs_{\src{emu}}$
%is a program that hardly maintains any state. (It only maintains a global
%counter that gets incremented every time it receives control.
%The counter is just used in a switch statement
%to decide which call/return command to execute next.)
%With fine-grained memory sharing, in contrast, 
%$\ctxs_{\src{emu}}$ has to mimic the actions
%that the given context $\ctxt_{\trg{given}}$ 
%does on the shared part of the memory.
%To understand how this need for mimicking shared memory arises,
%observe the difference (\ul{underlined}) between
%$\lambda_{\mi{prior\_work}}$ and
%our $\lambda$:
%\begin{align*}
%\lambda ::= \tau \mid \checkmark &\mid
%\mathtt{call}(\mi{fid}) ~\OB{v}~?~\text{\ul{\emph{Mem}, \emph{nalloc}}}
%\\
%&
%\mid
%\mathtt{call}(\mi{fid}) ~\OB{v}~!~\text{\ul{\emph{Mem}, \emph{nalloc}}}
%\\
%&
%\mid
%\mathtt{ret}~?~\text{\ul{\emph{Mem}, \emph{nalloc}}}
%% \\
%% &
%\mid
%\mathtt{ret}~!~\text{\ul{\emph{Mem}, \emph{nalloc}}}
%\end{align*}
%
%\Cref{sec:treq} explains this alphabet $\lambda$ in detail, but the key message here
%is that, with fine-grained memory sharing, the trace actions
%must (due to \Cref{soundness-target-trace-equivalence,completeness-source-trace-equivalence})
%carry a piece of memory $\mi{Mem}$ that represents a dump of 
%the content of all
%the memory locations that are shared so far.
%And to mimic such an action, $\ctxs_{\src{emu}}$ now 
%must write (every time it receives control) the same
%content to the same locations.
%This content can be capability values (i.e., unforgeable), 
%so these capability values cannot be
%(like prior work does for arguments and return values) hard-coded. Instead,
%what we do is we remember them by copying them to private memory.
%
%Thus, unlike in prior work, one now has to write invariants that govern the 
%private memory and the shared memory of the emulating context 
%$\ctxs_{\src{emu}}$ in order to be able to prove the \textbf{goal} above.
%Previous proofs never had to deal with proving such invariants.
%To add to this challenge, one has to use the information
%from \emph{Hypothesis 1} to argue that the mimicking that
%$\ctxs_{\src{emu}}$ does actually elicits the same action from
%the source program \src{p} as the action of \compilersymbol{\src{p}}
%under $\ctxt_{\trg{given}}$. For that, one would ideally want to
%use compiler correctness. Our proof technique, \tricl enables
%us indeed to use the information in \emph{Hypothesis 1} to instantiate
%\emph{whole-program compiler correctness} lemmas.
%
%\subsubsection{State of the art in reusing the compiler correctness lemmas}
%
%
%
%
%
%
%\todo[inline]{END: Think of a story}

%\subsection{Crucial Changes to the Main Theorem and to 
%\recombination}
%\label{sec:recombination}
%......

\subsection{Back-translation of data-flow traces}
\label{sec:data-flow-traces-detailed}

With memory sharing among components allowed
(in both target and source languages), the
observable trace events carry part of the state,
namely, the part of the memory that is shared so far.
To mimic such an event, one needs to mimic 
successful writes to memory. Mimicking the 
target-level memory writes
in the source program a) successfully
(i.e., without running into undefined behavior)
and b) without the need to do lots of book-keeping
of the necessary memory pointers is the 
key problem that \emph{data-flow traces} are designed
to solve. 

As mentioned in \Cref{sec:data-flow-traces}, we reduce
the problem of back-translating a trace of observable
events (namely, \Cref{lemma-robustptrs-backtrans}) 
to the problem of back-translating a trace
of all the data-flow events (a more informative trace
than the trace of just the observable events).
The reduction is straightforward since to begin with,
we define the trace semantics of observable events
in terms of the trace semantics of the data-flow events,
i.e., using an erasure/projection function that removes 
the extra information from the data-flow trace.

We argue that back-translating the more informative
trace is easier: informally, we think the data-flow
trace is a nice trade-off between syntax-directed
back-translation (which requires back-translating an
arbitrary target-language expression, including
for example unstructured control flow of the target language)
and the traditional trace-directed back-translation, which
usually requires setting up tedious invariants on
metadata that the mimicking source program has to
maintain.

Namely, in the traditional trace-directed back-translation,
we would need (as we did in \capableptrs) 
invariants that state that for
every value \src{v} that newly appeared (at a given trace position)
in an observable memory location \src{l},
there must
have existed two locations \src{l'_{l}}
and \src{l'_{v}}
in the private
memory of our mimicking source program such that 
there is a path from location \src{l'_{l}}
to a capability that authorizes the write
to \src{l} and a path from location \src{l'_{v}} to
the capability \src{v}---if \src{v} itself were
a capability value\footnote{More technically,
	it suffices that the location \src{l'_{v}} contains
	a capability value \src{v'} from which
	\src{v} can be derived.}. 

If such locations \src{l'_{l}} and \src{l'_{v}}
exist, then the mimicking program can traverse these
two paths in order
to mimic the change to location \src{l}.
Traversing the two paths means executing
an assignment command whose l-value and r-value
are each an expression that executes a 
sequence of memory accesses (i.e., array access
operators). Such an assignment (in C syntax) looks
as follows:
\src{^{*}(l'_{l}~[off_l^{1}][off_l^{2}]\ldots[off_l^n])\ 
	= l'_{v}~[off_v^{1}][off_v^{2}]\ldots[off_v^m];}.
However, maintaining the invariant described
above is inconvenient when the relation
between the memory of the mimicking program and the 
memory of the given target execution is not strong
enough. In particular, the memory relation says
nothing about the \emph{private} memory of the target 
context since this part of the memory is not part
of the observable events and the syntax of the target
context is not given either (just the trace).

To overcome the limitation of the memory relation
being too weak,
the workaround we used in \capableptrs is to
maintain a strong invariant between the memory of
the mimicking program and the 
\emph{entire history} 
of shared memories that appeared on
the trace prefix so far.
But to establish this strong invariant, we needed to
have the mimicking program do some book-keeping
functionality (see, e.g., the variables that
the example back-translation in
 \Cref{backtrans-example} keeps), which can become
 tedious to prove correct.

The correctness of the new construction
 (the back-translation
of data-flow traces) is arguably more convenient
because it does not require the tedious invariants 
mentioned above,
and because the simulation condition
needed for a big part of the invariant
is a lock-step simulation---thanks to the design of the 
alphabet of data flow events and the way
the source program is defined to simulate these 
events. The source program keeps one private 
memory location in sync with each
register in the target language. 
This finite set of private locations
is related in a lock-step simulation relation to
the register file.

\subsection{Related Work to \robustptrs}
\label{sec:robustptrs-relatedwork}

\subsubsection*{Other formal guarantees that are 
also referred to as compiler security}

There is a line of work
on understanding the space of possible security 
guarantees that one may want to
prove~\cite{abate2019journey,10.1145/3436809,DBLP:conf/esop/AbateBCD0HPTT20,patterson2019next}.....

There is also work on preserving constant-timeness.......

\subsubsection*{A History of Robust Safety}

The use of the word \emph{robust(ly)} in verification
literature first appeared in the title
``Robust Satisfaction'' 
by \citet{10.1007/3-540-48320-9_27}, in which they
coin the term
 to refer to the modular 
 model-checking problem, which was first proposed by 
\citet{grumberg1991model}. This mention of
the term was in the model checking literature, but
later on, \citet{gordon2003authenticity} would borrow
the word ``robust'' and use the term
``robust safety'' in the context of the spi-calculus,
and more recently, \citet{swasey2017robust} borrow the
latter term and use it to describe a desirable property
that a programming language has to satisfy in order
to support object capability patterns. Most recently,
\citet{10.1145/3371100} also use the term
\emph{robust safety} to refer to a language
feature they proved about a 
typed language that enables interactions with
untrusted but sandboxed code. The language feature
guarantees that any chosen system call policy
(a safety property) can be adhered to thanks to the
sandboxing features of the language.

\subsubsection*{Preservation of Robust Safety}

A line of work by \citet{rsc,10.1145/3436809} was the
first to propose preservation of robust safety as
an alternative compiler security criterion to 
compiler full abstraction. They argue that preservation
of robust safety can be more easily
(by choosing an appropriate trace relation)
and sometimes more efficiently
realized for realistic compilers whose source
and target languages potentially have an abstraction 
gap that would not easily tolerated by the compiler
full abstraction requirement.

\subsubsection*{Reuse of Whole-Program Compiler
Correctness Lemmas}

No work on syntax-directed
back-translation claims to
have reused \emph{whole-program} compiler correctness. 
With the trace-based approach though,
we are not the first to achieve reuse of whole-program 
compiler correctness,
but we are the first to achieve it while 
simultaneously supporting fine-grained memory sharing.
In \capableptrs, we already achieved this milestone.
In \robustptrs, we additionally use mechanized proofs.

The work by
\citet{Abate:2018:GCG:3243734.3243745} shows for the first time 
how one can reuse a \emph{whole-program} compiler correctness result 
(namely, compiler forward- and backward-simulation \`a la
\cite{Leroy2009}) in
the compiler 
security proof. This re-usability advantage is important. Many compiler 
security
results either happen to rely (as part of the proof) on some form of 
(e.g., compositional \cite{New}) compiler
correctness or even these results
(like condition \ref{condition-preserves} of 
\Cref{sec:background}) only 
become
meaningful (i.e., non-trivial) when accompanied with a compiler correctness 
result (like condition \ref{condition-reflects} of 
\Cref{sec:background}).
Thus, proving (some form of)
compiler correctness comes up almost always when 
proving
compiler security. And being able to reuse conventional (i.e., 
whole-program)
compiler correctness lemmas (rather than implicitly re-prove them) makes the
proofs modular and the proof techniques more promising for future 
verification efforts.
The main advantage of
 \citet{Abate:2018:GCG:3243734.3243745} compared to
other work \cite{10.1145/3436809} on proof techniques 
for instances of robust preservation 
\cite{abate2019journey}
is that it is a mechanized proof.

However, the work by \citet{Abate:2018:GCG:3243734.3243745}
makes the key simplifying
assumption that 
program
components do not share memory with each other. This prohibition of sharing
enables them to assume what is called "composition"
(see assumption 5 in 
\cite{Abate:2018:GCG:3243734.3243745}). 
In fact, their proof \cite{recombination-coq} of
this statement
relies heavily on the prohibition of sharing any C pointers 
across component boundaries.
In \robustptrs, we lift this prohibition, while 
maintaining
the proof reuse advantage.

==> technical-prelims.tex <==
% !TEX root = ./paper.tex

For both our source and target languages, we model two
runtime values

==> texdirectives.tex <==
\draftfalse\anonfalse\difffalse\appendixtrue

